Rectilinear Planarity Testing of Plane Series-Parallel Graphs in Linear Time

A plane graph is rectilinear planar if it admits an embedding-preserving straight-line drawing where each edge is either horizontal or vertical. We prove that rectilinear planarity testing can be solved in optimal $O(n)$ time for any plane series-parallel graph $G$ with $n$ vertices. If $G$ is rectilinear planar, an embedding-preserving rectilinear planar drawing of $G$ can be constructed in $O(n)$ time. Our result is based on a characterization of rectilinear planar series-parallel graphs in terms of intervals of orthogonal spirality that their components can have, and it leads to an algorithm that can be easily implemented.

==> app-rect-alg-sp.tex <==
			
\renewcommand{\arraystretch}{1.5}
\begin{table}[tb]
	\centering
	\scriptsize
	\caption{Running Example based on Figure~\ref{fi:prel}}\label{ta:runningexample}
%	\begin{tabular}{| c| c| c| c| c|}
%		\hline
%		$n$ & \textsc{Node Label} &  \textsc{Node Type} & \textsc{Children} & \textsc{Repres. Interval} &  \textsc{Spirality in $H$} \\
%		\hline
%		 
%		\hline
%		
%		\hline
%	\end{tabular} 
\end{table}


